Comparing the behavior of OpenMP Implementations with various Applications on two different Fujitsu A64FX platforms

The development of the A64FX processor by Fujitsu has been a massive innovation in vectorized processors and led to Fugaku: the current world's fastest supercomputer. We use a variety of tools to analyze the behavior and performance of several OpenMP applications with different compilers, and how these applications scale on the different A64FX processors on clusters at Stony Brook University and RIKEN.

==> sections/conclusions.tex <==
In this paper, we have studied and observed the behavior of OpenMP
implementations
on the A64FX processor across several applications and several compiler toolchains. We have also analyzed how these applications run on both a standard
 % TONY RedHat
 CentOS
 Linux distribution and compared it to that of a stripped-down and customized Linux kernel. We have observed that Cray's compilers and GNU/LLVM compilers that have support for ARM-based processors appear to scale better with OpenMP compared to the Fujitsu compilers. We have observed that, while having the most optimal performance, the Cray Compilers may generate incorrect instructions, such as with the Minimod application, leading to incorrect results. 
  % TONY: not sure I understand.  Isn't this more to do with the MPI implementation?
 % Honestly, I'm not sure. Tetsuya's replies to my messages didn't indicate anything about MPI implementation having an effect, only that OpenMP doesn't scale well across CMG's
 % You can't say "OpenMP doesn't scale well" you have to talk about the behavior of individual implementations.
 
Moving forward, we wish to explore more complex OpenMP behavior, including shared address spaces between threads, examining in-depth behavior of thread over-subscription and what can be done to mitigate it on the A64FX processor. In addition, examining how the Fujitsu compiler toolchain behaves on Ookami would make an interesting comparison with how it functions on Fugaku, similar to comparing GNU's Compiler performance on both clusters, in addition to measuring metrics on Ookami through Fujitsu's profiling tools.

